GRAPE: Generalizable and Robust Multi-view Facial Capture

Deep learning-based multi-view facial capture methods have shown impressive accuracy while being several orders of magnitude faster than a traditional mesh registration pipeline. However, the existing systems (e.g. TEMPEH) are strictly restricted to inference on the data captured by the same camera array used to capture their training data. In this study, we aim to improve the generalization ability so that a trained model can be readily used for inference (i.e. capture new data) on a different camera array. To this end, we propose a more generalizable initialization module to extract the camera array-agnostic 3D feature, including a visual hull-based head localization and a visibility-aware 3D feature aggregation module enabled by the visual hull. In addition, we propose an ``update-by-disagreement'' learning strategy to better handle data noise (e.g. inaccurate registration, scan noise) by discarding potentially inaccurate supervision signals during training. The resultant generalizable and robust topologically consistent multi-view facial capture system (GRAPE) can be readily used to capture data on a different camera array, reducing great effort on data collection and processing. Experiments on the FaMoS and FaceScape datasets demonstrate the effectiveness of the proposed method.

==> tabs_and_figs/fig_teaser.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{images/teaser.pdf}
\caption{Our model trained on one dataset can be directly used on another dataset (i.e. data captured by a different camera array) and produces pretty accurate results (1.7 mm), surpassing TEMPEH (failed) and DECA by a large margin.
The capability greatly reduces the data collection (e.g. 95 subjects, 28 expressions for each subject, 97946 frames in total~\cite{tempeh}) and processing effort when building a new camera array.}
\label{fig:teaser}
\end{figure}

==> tabs_and_figs/tab_domain_adapt_FS2FMS.tex <==
\begin{table}[t]
\scriptsize
    \caption{\textbf{Model generalization}. The models are trained on the FaceScape dataset and evaluated on the FaMoS dataset. Errors in mm.
    }
    \label{tab:generalization_facescape_famos}
    \centering
    \begin{tabular}{l|rrr|rrr|rrr}
    \toprule
           & \multicolumn{3}{c|}{w/o fine-tune. } &  \multicolumn{3}{c|}{Subj. A} &  \multicolumn{3}{c}{Subj. B} \\
           Method (FS $\rightarrow$ FaMoS) & Median & Mean & Std & Median & Mean & Std & Median & Mean & Std \\
    \midrule

 TEMPEH global & 25.63 & 32.26 & 21.77 \\
 + occ init & 8.27 & 13.72 & 18.09 \\
 + vis & 15.52 & 30.21 & 28.59 \\
 \sysname{} global & 1.70 & 1.91 & 1.03 & \\
\sysname{} & 1.21& 1.41 & 1.03 \\

    \bottomrule
    \end{tabular}
\end{table}

==> tabs_and_figs/tab_famos_and_FS_combined.tex <==
\begin{table}[t]
\scriptsize
\caption{\textbf{Results on the combined dataset}. The models are trained on both the FaMoS training set and the FaceScape training sets.
Face region errors (in mm) are reported on their test sets separately.
}
\label{tab:sota_combine}
\vspace{-4mm}
\centering
\begin{tabular}{l|l|rrr|rrr}
\toprule
  & & \multicolumn{3}{c|}{FaMoS} &  \multicolumn{3}{c}{FaceScape} \\
 \midrule 
& Method & Med. & Avg. & Std. & Med. & Avg. & Std. \\
\midrule
a.1 & TEMPEH~\cite{tempeh} global & 5.65 & 6.70 & 4.01 & 8.50 & 12.15 & 9.01 \\
a.2 & \sysname{} global & 1.07 & 1.15 & 0.40 & 1.11& 1.25 & 0.39 \\
\bottomrule
\end{tabular}
\end{table}
